Enhancing Contention Resolution ALOHA using Combining Techniques

Recently, random access protocols have acquired a new wave of interest, not only from the satellite communication community, but also from researchers active in fields like Internet of Things and machine-to-machine. Asynchronous (slot- and frame-wise) ALOHA-like random access protocols, are very attractive for such applications, enabling low complexity transmitters and avoiding time synchronization requirements. Evolutions of ALOHA employ time diversity through proactive replication of packets, but the time diversity is not fully exploited at the receiver. Combining techniques, as selection combining and maximal-ratio combining, are beneficial and are adopted in the enhanced contention resolution ALOHA (ECRA) scheme, presented here. A tight approximation of the packet loss rate for asynchronous random access, including ECRA, well suited for the low channel load region is derived. Finally, ECRA is evaluated in terms of spectral efficiency, throughput and packet loss rate in comparison with recent protocols, showing that it is able to largely outperform both slotted synchronous and asynchronous schemes.

==> 9-Acknowledgments/Acknowledgements.tex <==
\section{Acknowledgements}

==> sections/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% abbreviations.bib
%%%
%%% \acresetall resets all acronyms to not used. Useful after the abstract to redefine all acronyms in the introduction.
%%% \acf{label} Full: written out form with acronym in parentheses, irrespective of previous use
%%% \acs{label} acronym form, irrespective of previous use
%%% \acl{label} written out form without following acronym
%%% \acp{label} plural form of acronym by adding an s. \acfp. \acsp, \aclp work as well.
%%% \acs{label} Short: short version of the acronym
%%% \acfp, acsp aclp acfi acused acsu aclu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{acronym}
% A
\acro{A/A}{air-to-air}%
\acro{A-EXEC}{auto execute COCR service}%
\acro{AAC}{airline administrative control}%
\acro{ACK}{acknowledgement}%
\acro{ACP}{aeronautical communications panel}%
\acro{AF}{assured forwarding}%
\acro{AL}{application layer}%
\acro{ANSP}{air navigation service provider}%
\acro{AOC}{airline operational control}%
\acro{APC}{air passenger communication}%
\acro{APT}{airport}%
\acro{ATC}{air traffic control}%
\acro{ATI}{access technology independent}%
\acro{ATM}{air traffic management}%
\acro{ATN}{aeronautical telecommunication network}%
\acro{ATN/IPS}{aeronautical telecommunication network / internet protocol suite}%
\acro{ATN/OSI}{aeronautical telecommunication network / open systems interconnection reference model}%
\acro{ATS}{air traffic services}%
\acro{ATSC}{air traffic service communication}%
\acro{AVBDC}{absolute volume based dynamic capacity}%
\acro{AWGN}{additive white gaussian noise}%
% B
\acro{BB}{bandwidth broking} %
\acro{BBFRAME}{baseband frame}%
\acro{BE}{best effort}%
\acro{BER}{bit error rate}%
\acro{BGAN}{broadband global area network}%
\acro{BSM}{broadband satellite multimedia}%
% C
\acro{CA}{constrained architecture}%
\acro{CAC}{connection admission Control}%
\acro{CC}{congestion control}%
\acro{CDF}{cumulative distribution function}
\acro{CDMA}{code divison multiple access}%
\acro{CLNP}{connectionless networking protocol}%
\acro{CLTP}{connectionless transport protocol}%
\acro{CoA}{care of address}%
\acro{CoS}{class of service}%
\acro{COCR}{communications operating concept and requirements for the future radio system}%
\acro{COTP}{connection oriented transport protocol}%
\acro{COTS}{commercial-off-the-shelf}%
%%\acro{CRA}{Constant Rate Assignment}%
\acro{CRA-CC}{CRA-convolutional code}%
\acro{CRA-SH}{CRA-shannon bound}%
\acro{CRA}{contention resolution ALOHA}%
\acro{CRC}{cyclic redundancy check}%
\acro{CRDSA}{contention resolution diversity slotted ALOHA}%
\acro{CRDSA++}{contention resolution diversity slotted ALOHA++}%
\acro{CS}{class selector}%
\acro{CSA}{coded slotted ALOHA}%
\acro{CSMA}{carrier sense multiple access}%
% D
\acro{DAMA}{demand assigned multiple access}%
\acro{DiffServ}{differentiated services}%
\acro{DoD}{department of defence}%
\acro{DSA}{diversity slotted ALOHA}%
\acro{DSCP}{diffServ code point}%
\acro{DVB}{digital video broadcasting}%
\acro{DVB-RCS+M}{digital video broadcasting - return channel via satellite mobility}%
\acro{DVB-RCS}{digital video broadcasting - return channel via satellite}%
\acro{DVB-S2}{digital video broadcasting - second generation}%
\acro{DVB-S2/RCS}{digital video broadcasting - second generation / return channel via satellite}%
% E
\acro{ECN}{explicite congestion notification}%
\acro{ECRA}{enhanced contention resolution ALOHA}%
\acro{ECRA-SC}{ECRA selection combining}
\acro{ECRA-MRC}{ECRA maximal ratio combining}
\acro{ECTL}{eurocontrol}%
\acro{EF}{expedited forwarding}%
\acro{EGD}{equal-gain diversity}
\acro{ENR}{en-route}%
\acro{ES}{end system}%
\acro{ESA}{European space agency}%
\acro{ETSI}{European telecommunications standards institute}%
\acro{ETSI-BSM}{European telecommunications standards institute - broadband satellite multimedia}%
% F
\acro{FAA}{federal aviation administration}%
\acro{FCA}{free capacity assignment}%
\acro{FDM}{frequency division multiplexing}%
\acro{FDMA}{frequency division multiple access}%
\acro{FEC}{forward error correction}%
\acro{FET}{first entry times}%
\acro{FL}{forward link}%
% G
\acro{GEO}{geostationary orbit}%
\acro{GIG}{global information grid}%
\acro{GSE}{generic stream encapsulation}%
% H
\acro{HA}{home agent}%
\acro{HF}{high frequency}%
% I
\acro{IC}{interference cancellation}%
\acro{ICAO}{international civil aviation organization}%
\acro{IETF}{internet engineering task force}%
\acro{IntServ}{integrated services}%
\acro{IP}{internet protocol}%
\acro{IPS}{internet protocol suite}%
\acro{IPSec}{IP security}%
\acro{IRCRA}{irregular repetition contention resolution ALOHA}%
\acro{IRSA}{irregular repetition slotted ALOHA} %
\acro{IS}{intermediate system}%
\acro{IS-IS-TE}{intermediate system to intermediate system extension for traffic engineering}%
\acro{ISI}{input stream identifier}%
\acro{ISO/OSI}{international organization for standardization/open systems interconnection}%
% K
\acro{Ku}{kurz-under}%
\acro{Ka}{kurz-above}%
% L
\acro{LAE}{link access equipment}%
\acro{LAN}{local area network}%
\acro{LD}{low density}%
\acro{LDACS}{L-band digital aeronautical communication system}%
\acro{L-DACS}{L-band digital aeronautical communication system}%
\acro{LDPC}{low density parity check codes}%
\acro{LEO}{low earth orbit}%
% M
\acro{M2M}{machine-to-machine}
\acro{MAC}{medium access}%
\acro{MCAST}{multicast}%
\acro{MF-TDMA}{multifrequency time division multiple access}%
\acro{MH}{mobile host}%
\acro{MIHF}{Media independent handover function}%
\acro{MLPP}{multi level priority preemption}%
\acro{Mode-S}{mode-select}%
\acro{MPE}{multi protocol encapsulation}%
\acro{MPEG2-TS}{MPEG2 - transport stream}%
\acro{MPLS}{multi protocol label switching}%
\acro{MRC}{maximal-ratio combining}
% N
\acro{NCC}{network control centre}%
\acro{NET}{network connectivity}
\acro{NEWSKY}{NEtWorking the SKY for aeronautical communications}%
\acro{NOC}{non-operational communication}%
\acro{NSIS}{next steps in signalling}%
% O
\acro{OC}{operational communication}%
\acro{ORP}{oceanic, remote and polar}%
\acro{OSI}{open systems interconnection}%
\acro{OSPF}{open shortes path first}%
% P
\acro{PDF}{probability density function}%
\acro{PCE}{predictive capacity estimation}%
\acro{PCN}{pre-congestion notification}%
\acro{PDU}{protocol data unit}%
\acro{PEP}{performance enhancing proxy}%
\acro{PER}{packet error rate}%
\acro{PID}{packet identifier}%
\acro{PLFRAME}{physical layer frame}%
\acro{PLR}{packet loss rates}%
% Q
\acro{QoS}{quality of service}%
\acro{QoS-PRN}{QoS private relay nodes}%
\acro{QoS-RN}{QoS-relay nodes}%
% R
\acro{RA}{random access}%
\acro{RBDC}{rate based dynamic capacity}%
\acro{RCB}{random coding bound}%
\acro{RCS}{return channel via satellite}%
\acro{RCS+M}{return channel via satellite plus mobility}%
\acro{RF}{radio frequency}%
\acro{RFC}{request for comments}%
\acro{RL}{return link}%
\acro{RM}{resource management}%
\acro{RN}{relay nodes}%
\acro{RRM}{radio resource management}%
\acro{RS}{reed solomon}%
\acro{RSVP}{resource reservation protocol}%
\acro{RTT}{round trip time}%
% S
\acro{SA}{slotted ALOHA}%
\acro{SANDRA}{seamless aeronautical networking through integration of data links, radios and antennas}%
\acro{SB}{Shannon bound}%
\acro{S2}{second generation}%
\acro{SC}{selection combining}
\acro{SESAR}{single European sky ATM research}%
\acro{SF}{superframe}%
\acro{SIC}{successive interference cancellation}%
\acro{SLS}{service level specification}%
\acro{SNDCF}{subnetwork dependent convergence function}%
\acro{SNIR}{signal-to-noise and interference ratio}%
\acro{SNR}{signal-to-noise ratio}%
\acro{SWIM}{system wide information management}%
\acro{SYN}{synchronization}%
\acro{SYNC}{synchronization}%
% T
\acro{TCP}{transport control protocol}%
\acro{TCP/IP}{transport control protocol / internet protocol suite}%
\acro{TDMA}{time division multiple access}%
\acro{TE}{traffic engineering}%
\acro{TI}{technology independent}%
\acro{TI-SAP}{technology independent - service access point}%
\acro{TD}{technology dependent}%
\acro{TL}{transport layer}%
\acro{TMA}{terminal maneuvering area}%
\acro{ToS}{type of service}%
% U
\acro{UCA}{unconstrained architecture}%
\acro{UDP}{user datagram protocol}%
% V
\acro{VBDC}{volume based dynamic capacity}%
\acro{VDL}{VHF digital mode}%
\acro{VHF}{very high frequency}%
\acro{VoIP}{voice over IP}%
\acro{VPN}{virtual private networks}%
% W
\acro{WG}{working group}%
\acro{WiMAX}{worldwide interoperability for microwave access}%
% X
\acro{XFECFRAME}{forward error correction frame}%
\end{acronym}

\makeatletter
\newif\ifAC@uppercase@first
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}
\def\AC@aclp#1{%
  \ifcsname fn@#1@PL\endcsname
    \ifAC@uppercase@first
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname
    \else
      \csname fn@#1@PL\endcsname
    \fi
  \else
    \AC@acl{#1}s
  \fi 
}
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}
\def\AC@acrodef#1[#2]#3{%
  \@bsphack
  \protected@write\@auxout{}{%
    \string\newacro{#1}[#2]{\AC@uppercase@write #3}%
  }\@esphack
}
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\makeatother


==> sections/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\tp$ & \verb;\tp; & Throughput \\
$\se$ & \verb;\se; & Spectral Efficiency \\
$\plr$ & \verb;\plr; & Packet Loss Rate \\
$\rate$ & \verb;\rate; & Rate \\
$\maxRate$ & \verb;\maxRate; & Maximum Rate allowed\\
$\mutInf$ & \verb;\mutInf; & Mutual information\\
$\rvDec$ & \verb;\rvDec; & r.v. denoting the outcome of the decoding process\\
$\capacity$ & \verb;\capacity; & Capacity \\
$\capacitySC$ & \verb;\capacitySC; & Capacity selection combinig\\
$\capacityMRC$ & \verb;\capacityMRC; & Capacity maximal-ratio combining\\
$\refCap$ & \verb;\refCap; & Reference Capacity of the Gaussian MAC \\
$\maxCap$ & \verb;\maxCap; & Maximum Capacity \\
$\maxSe$ & \verb;\maxSe; & Maximum spectral efficiency \\
$\normCap$ & \verb;\normCap; & Normalized capacity \\
\\
$\dg$ & \verb;\dg; & Number of replicas per user, i.e. degree \\
\\
$\fraLen$ & \verb;\fraLen; & VF duration \\
$\pkLen$ & \verb;\pkLen; & Packet duration \\
$\symLen$ & \verb;\symLen; & Symbol duration \\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\fraTp$ & \verb;\fraTp; & Duration of VF in packets durations \\
$\VFStart$ & \verb;\VFStart; & Delay w.r.t. the VF start \\
$\RefTime$ & \verb;\RefTime; & User delay w.r.t. the common reference time \\
$\Wind$ & \verb;\Wind; & Decoder window size \\
$\WindSh$ & \verb;\WindSh; & Decoder window shift \\
\\
$\numUs$ & \verb;\numUs; & number of user/transmission terminals \\
$\numSym$ & \verb;\numSym; & number of symbols in a packet/replica \\
$\numBit$ & \verb;\numBit; & number of information bits per packet/replica \\
\\
$\rx$ & \verb;\rx; & received signal \\
$\rxVec$ & \verb;\rxVec; & vector of received samples/symbols \\
$\tx$ & \verb;\tx; & transmitted signal \\
$\txVec$ & \verb;\txVec; & vector of transmitted samples/symbols \\
$\noise$ & \verb;\noise; & noise signal \\
$\noisePr$ & \verb;\noisePr; & white Gaussian process \\
$\noiseVec$ & \verb;\noiseVec; & vector of noise samples \\
$\noiseVar$ & \verb;\noiseVar; & noise variance \\
$\intVal$ & \verb;\intVal; & interference random variable \\
$\intVec$ & \verb;\intVec; & vector of interference samples \\
$\intNum$ & \verb;\intNum; & number of interferers \\
$\ch$ & \verb;\ch; & channel amplitude \\
$\symVal$ & \verb;\symVal; & value of the transmitted symbol \\
$\pulse$ & \verb;\pulse; & pulse shape raised cosine filter \\
$\pulseRoot$ & \verb;\pulseRoot; & pulse shape root raised cosine filter \\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\tm$ & \verb;\tm; & time \\
$\epoch$ & \verb;\epoch; & epoch \\
$\freq$ & \verb;\freq; & frequency \\
$\phase$ & \verb;\phase; & phase \\
\\
$\user$ & \verb;\user; & user index \\
$\replica$ & \verb;\replica; & replica index \\
$\sym$ & \verb;\sym; & symbol index \\
\\
$\usPw$ & \verb;\usPw; & useful received power \\
$\PwAg$ & \verb;\PwAg; & Aggregated recevied power \\
$\usPwTx$ & \verb;\usPwTx; & User transmission power \\
$\noisePw$ & \verb;\noisePw; & noise power \\
$\noiseSD$ & \verb;\noiseSD; & single-sided noise power spectral density \\
$\intPw$ & \verb;\intPw; & interference power \\
$\sinr$ & \verb;\sinr; & \ac{SINR} \\
$\sinrVec$ & \verb;\sinrVec; & \ac{SINR} vector \\
\\
$\UCP$ & \verb;\UCP; & Index of a given \ac{UCP} \\
$\UCPcons$ & \verb;\UCPcons; & Considered \ac{UCP} \\
$\AllUCP$ & \verb;\AllUCP; & Set of all possible \ac{UCP} \\
$\Code$ & \verb;\Code; & Code selected \\
$\CollClus$ & \verb;\CollClus; & Collision Cluster \\
\hline \hline
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\RStart$ & \verb;\RStart; & Start time of a replica \\
$\VL$ & \verb;\VL; & Left shift w.r.t. to the replica start where the Vulnerable period starts \\
$\VR$ & \verb;\VR; & Right shift w.r.t. to the replica start where the Vulnerable period ends \\
$\Vg$ & \verb;\Vg; & For the asynchronous protocols, symmetric time shift \\
$\Vpd$ & \verb;\Vpd; & Vulnerable period duration \\
$\nVp$ & \verb;\nVp; & Number of vulnerable periods per \ac{VF} \\
\\
$\mU$ & \verb;\mU; & Number of possible selections of 2 users out of m \\
$\sL$ & \verb;\sL; & Number of ways to select slots in $\UCPcons$ \\
$\UL$ & \verb;\UL; & Number of ways to select slots in $\UCPcons$ for two users \\
\\
$\intFreeAsy$ & \verb;\intFreeAsy; & Fraction of interference free replica for async. RA \\
$\intFreeMRC$ & \verb;\intFreeMRC; & Fraction of interference free replica for RA after MRC \\
$\intOne$ & \verb;\intOne; & Portion of combined observation interfered only in one portion  \\
$\rateFree$ & \verb;\rateFree; & Rate corresponding to the interference free part of the replica \\
$\rateInt$ & \verb;\rateInt; & Rate corresponding to the interfered part of the replica \\
$\rateIntO$ & \verb;\rateIntO; & Rate corresponding to the interfered part of the replica \\
$\rateIntT$ & \verb;\rateIntT; & Rate corresponding to the interfered part of the replica \\
\\
\hline \hline
\end{tabular}
\end{center}







\clearpage 

==> sections/preamble.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand{\fede}[1]{\textcolor{red}{#1}}
\newcommand{\giangio}{\textcolor{blue!80}}
\newcommand{\andrea}{\textcolor{green!80}}

%%%% Notation

\newcommand{\ET}{\mathrm{E}_T}    %% Tx energy
\newcommand{\EL}{\mathrm{E}_L}    %% Listen energy
\newcommand{\EI}{\mathrm{E}_I}    %% Idle energy
\newcommand{\E}{\mathrm{E}}		  % % Total average energy


\newcommand{\La}{\Lambda}    %% Node oriented dd (user)
\newcommand{\Rh}{\mathrm{P}}    %% Node oriented dd (slot)
\newcommand{\la}{\lambda}    %% edge oriented dd (user)
\newcommand{\rh}{\rho}    %% egde oriented dd (slot)

\newcommand{\iLa}[1]{\Lambda^{(#1)}}    %% Induced Node oriented dd (user)
\newcommand{\iRh}[1]{\mathrm{P}^{(#1)}}    %% Induced  Node oriented dd (slot)
\newcommand{\ila}[1]{\lambda^{(#1)}}    %% Induced edge oriented dd (user)
\newcommand{\irh}[1]{\rho^{(#1)}}    %% Induced  egde oriented dd (slot)

\newcommand{\graph}{\mathscr{G}}    %% Graph
\newcommand{\uset}{\mathscr{U}}    %% user nodes set
\newcommand{\sset}{\mathscr{S}}    %% slot nodes set
\newcommand{\listset}{\mathscr{L}}    %% listen set
\newcommand{\sn}{\mathsf{s}}    %% listen set
\newcommand{\un}{\mathsf{u}}    %% listen set


\newcommand{\dum}{\mathtt{x}}    %% dummy variable

\newcommand{\load}{\mathsf{G}}    %% channel load
\newcommand{\thrp}{\mathsf{R}_{\mathrm{D}}}    %% throughput
\newcommand{\plr}{\mathsf{P}_{\mathrm{MD}}}    %% PLR

\newcommand{\thr}{\mathsf{G}^\star}    %% threshold
\newcommand{\plrt}{\plr^\star}    %% PLR

\newcommand{\slots}{n} % % number of slots per discovery phase
\newcommand{\tslot}{\mathrm{T}_s} % % number of slots per discovery phase
\newcommand{\users}{m} % % number of users in the network

\newcommand{\degree}{d} % % number of replicas sent per user, i.e. degree
\newcommand{\listn}{\ell} % % listening probability
\newcommand{\dmax}{{\degree_{\mathrm{max}}}}    %% Node oriented dd (user)
\newcommand{\avgd}{\bar\degree}    %% Node oriented dd (user)

\newcommand{\dcost}{\mathrm{D}_C}    %% Node oriented dd (user)


\newcommand\T{\rule{0pt}{2.6ex}}

